What Makes Training Multi-Modal Classification Networks Hard?

Consider end-to-end training of a multi-modal vs. a single-modal network on a task with multiple input modalities: the multi-modal network receives more information, so it should match or outperform its single-modal counterpart. In our experiments, however, we observe the opposite: the best single-modal network always outperforms the multi-modal network. This observation is consistent across different combinations of modalities and on different tasks and benchmarks. This paper identifies two main causes for this performance drop: first, multi-modal networks are often prone to overfitting due to increased capacity. Second, different modalities overfit and generalize at different rates, so training them jointly with a single optimization strategy is sub-optimal. We address these two problems with a technique we call Gradient Blending, which computes an optimal blend of modalities based on their overfitting behavior. We demonstrate that Gradient Blending outperforms widely-used baselines for avoiding overfitting and achieves state-of-the-art accuracy on various tasks including human action recognition, ego-centric action recognition, and acoustic event detection.

==> related_work.tex <==
\section{Related Work} \label{sec:related_work}

Our work is related to the previous line of research on multi-modal networks~\cite{Baltruaitis2018MultimodalML} for classifications~\cite{SimonyanZ14,WangXW0LTG16,FeichtenhoferPZ16,Fukui16,I3D,Arevalo17,abs-1708-03805,Kiela18}, which primarily uses pre-training in contrast to our joint training. On the other hand, our work is also related to cross-modal tasks~\cite{Weston:2011:WSU:2283696.2283856,NIPS2013_5204,Socher:2013:ZLT:2999611.2999716,VQA,balanced_binary_vqa,balanced_vqa_v2,ImageCaption16} and cross-modal self-supervised learning~\cite{ZhaoSOP18,L3Net17,Owens_2018_ECCV,Korbar18}. These tasks either take one modality as input and make prediction on the other modality (e.g. Visual-Q\&A\cite{VQA,balanced_binary_vqa,balanced_vqa_v2}, image captioning~\cite{ImageCaption16}, sound localization~\cite{Owens_2018_ECCV,ZhaoSOP18} in videos) or uses cross-modality correspondences as self-supervision (e.g. image-audio correspondence~\cite{L3Net17}, video-audio synchronization~\cite{Korbar18}). Different from them, our Gradient-Blending tries to address the problem of joint training of multi-modal for classification. The Gradient-Blending training scheme is also related to other works on auxiliary loss, which is widely adopted in multi-task learning approaches~\cite{Kokkinos16,Eigen15,Kendall18,GradNorm18}. These methods either use uniform\textbackslash manually tuned weights, or learn the weights as parameters during training, while our work re-calibrates supervision signals using \textit{a prior} \emph{OGR}.

% On one hand, many tasks require more than one modality to accomplish, such as Visual-Question-Answering (VQA) \cite{VQA,balanced_binary_vqa,balanced_vqa_v2} and image captioning \cite{ImageCaption16}; or they use one modality as supervision signal for the other (self-supervised learning) \cite{ZhaoSOP18,L3Net17,Owens_2018_ECCV,Korbar18}. These tasks cannot be performed without multi-modal networks. On the other hand, many tasks can be done with a single-modal network, but the task is multi-modal, such as video classifications \cite{SimonyanZ14,WangXW0LTG16,FeichtenhoferPZ16,I3D} and image plus text classifications \cite{Arevalo17,Kiela18}. Our work is more related to the second stream, where the task can be performed by a single-modal network while more than one modalities are available as inputs. Instead of using pre-training, either on the same or a different datasets as aforementioned works, our work focuses on how to train the network jointly. Although our paper uses the default fusion method by concatenation, some orthogonal works provide new fusion architectures \cite{Fukui16,Arevalo17,Owens_2018_ECCV,Kiela18}, and we believe our method is applicable to other fusion strategies as well.  


